Revisiting migration in a disc cavity to explain the high eccentricities of warm Jupiters

The distribution of eccentricities of warm giant exoplanets is commonly explained through planet--planet interactions, although no physically sound argument favours the ubiquity of such interactions. No simple, generic explanation has been put forward to explain the high mean eccentricity of these planets. In this paper, we revisit a simple, plausible explanation to account for the eccentricities of warm Jupiters: migration inside a cavity in the protoplanetary disc. Such a scenario allows to excite the outer eccentric resonances, a working mechanism for higher mass planets, leading to a growth in the eccentricity while preventing other, closer resonances to damp eccentricity. We test this idea with diverse numerical simulations, which show that the eccentricity of a Jupiter-mass planet around a Sun-like star can increase up to 0.4, a value never reached before with solely planet--disc interactions. This high eccentricity is comparable to, if not larger than, the median eccentricity of warm Saturn- to Jupiter-mass exoplanets. We also discuss the effects such a mechanism would have on exoplanet observations. This scenario could have strong consequences on the discs lifetime and the physics of inner disc dispersal, which could be constrained by the eccentricity distribution of gas giants.

==> vieille_into <==
\section{Introduction}
% ===============
\label{sec:introduction}
It is now clear that exoplanets exhibit a much wider distribution of eccentricities and \cb{stellar obliquities} than \cb{the} planets of our solar system, and understanding why there is such a diversity is paramount to better constrain planetary formation and evolution. \cb{(CB: why 'now'? how about simply starting by 'Exoplanets exhibit...'?)}
% One of the possible explanation is that planets across the galaxy have extremely different 
% interactions with their protoplanetary disk during the early phases of their stellar system. 
For low-mass planets, a few times the mass of the Earth at most, \citet{Fromenteau2019} have recently emphasised the need to better understand the thermal feedback from the planet onto the surrounding gas \corr{(i.e. the heating of the disc due to the accretion luminosity of the planet)}. They have shown that there exists a critical accretion luminosity above which the usual paradigm that low mass planets migrate inward with a damping of their eccentricity and inclinations breaks. Above this luminosity, planets can experience an exponential increase of their eccentricity and migrate outwards. Such an explanation, however, is not valid for high-mass planets which carve a gap \cb{in their protoplanetary} disc (see review in, e.g., \citealp{Baruteau2013}). \cb{(CB: the transition between the first two sentences in this paragraph looks a little abrupt to me. Maybe you should state what level of eccentricity super-Earths / hot Neptunes can typically reach before suggesting a scenario that could account for some increase in eccentricity?)}

The commonly admitted theory to explain the high eccentricities of high mass planets, superior to $\sim 3 M_\mathrm{J}$ with $M_\mathrm{J}$ the mass of Jupiter, dates as back as 2001 with the work of \citet{Papaloizou2001}. They showed that high-mass planets \cb{on} circular orbits carve wide enough gaps in the disk \cb{(caution: disk or disc throughout the text, but not both!)} around their radial position to incorporate all the first-order Lindblad resonances, located within $\sim 1.58 r_\mathrm{p}$ with $r_\mathrm{p}$ the radial position of the planet, inside the gap. In that regard, all these resonances have an almost null effect on the torque exerted by the disk on the planet and the evolution of the \cb{planet's} orbital parameters is given by the next, most important resonance\cb{s}: the first-order eccentric resonance\cb{s}. \cb{They} lead to an exponential growth of the eccentricity, eventually controlled by the excitation of new eccentric resonances that oppose this eccentric instability. \cb{(is this really 'oppose' that you mean here? Like in the previous paragraph a few words on the typical eccentricity of warm Jupiters may be desirable. I don't think this would 'spoil' Figure 1 since it is well known that the medial eccentricity of warm Jupiters is about 0.25 or so -- we can work out a proper reference.)}

There is \cb{still, however,} outstanding questions regarding the eccentricity distribution of intermediate mass planets, between a few tens of the mass of the Earth to a few Jupiter masses. Recent theories \citep[see e.g.,][]{Anderson2019} need to invoke planet--planet scattering (see review in \citet{Armitage2011} ), although as stated by \citet{Armitage2011}, "there is no straightforward independent argument that the [...] initial conditions needed for [planet--planet scattering] to work are generically realized in nature". Therefore, planet--planet scattering appears to be a circumstantial explanation rather than a fundamental, general situation. 

In Figure \ref{fig:histo}, we show the \cb{eccentricity distribution of exoplanets} as a function of the ratio of their mass to the mass of their star, $q$, for planets with orbital period superior to 30 days. This histogram exhibits three distributions: for $q$ inferior to $ \sim 10^{-4}$, eccentricities are low and there are only few high- eccentricity ($> 0.4$) planets. For $10^{-4}<q<10^{-2.5}$, the distribution of eccentricities is sparser and the median is higher, around $0.25$. For higher $q$ \cb{values}, the low eccentricity bins empty out because of the mechanism proposed by \citet{Papaloizou2001}, preventing the existence of non-eccentric planets. \cb{(Does this mean the secondaries help carving the required cavity?)}

% FFFFFFFFFF
\begin{figure}
\centering
\includegraphics[width=\hsize]{Figures/histo_ecc_3.pdf}
\caption{\cb{Eccentricity distribution} of exoplanets as a function of the ratio of their mass to the mass of their star, $q$. The sum of the \cb{bin} values \cb{in} each column is one. All planets have an orbital period superior to 30 days to filter out planet\cb{s} circularized by star--planet tidal interactions. \cb{Data taken from \url{exoplanets.org}.} \cb{CB: please don't forget to add x-, y- and z-titles in this plot!}}
\label{fig:histo}
\end{figure}
% FFFFFFFFFF

Recent works have tried to explain the eccentricities of intermediate mass planets, $10^{-3.5}<q<10^{-2.5}$, from planet--disc interaction (e.g., \citealp{Rice2008,Dunhill2013,Bitsch2013,Rosotti2017}). The overall conclusion is that planet disc interactions tend to damp the eccentricity $e$ to small values ($e \lesssim 0.03$). \corr{\citet{Dangelo2006} obtained higher value for $e$ for Jupiter mass planets, although no other work have reached 
such high eccentricity, but they still conclude that it might not be sufficient to get to $e \sim 0.25$}. The outstanding question therefore remains: how can we explain the eccentricity distribution of intermediate mass planets? 

\citet{Duffell2015} have shown that Jupiter-like planets on fixed orbits can experience an increase in their eccentricity due to disc--planet interactions, which gets a limiting value of $\sim 0.07$ because of supersonic shocks with non eccentric gas. \corr{Their method can be discussed as a proper evolutionary scenario would be needed to assess their conclusion, and they neglect
the indirect term in the gravitational potential. Nonetheless,} they show that if eccentric motions in the discs are not favoured, contrary to the \citet{Papaloizou2001} case, the planet eccentricity experience a decrease due to shocks with the surrounding gas. \cb{isn't the previous sentence somewhat too long?} \corr{IS that better ?}. A mechanism which would increase strongly the eccentricity of an intermediate mass planet through disc interactions therefore needs to overcome the dissipated power through these shocks. 

Motivated by this realization, in this paper we propose a simple plausible explanation for the eccentricity of Jupiter mass planets: migration inside a cavity. If a cavity already exists in the inner part of the disk and the planet eventually migrates inside the cavity, the exponential increase of the eccentricity proposed by \citet{Papaloizou2001} can be triggered while supersonic shocks would not prevent eccentricity growth as seen in \citet{Duffell2015}, because the density inside the cavity is too low.

\corr{At the linear order, \citet{Teyssandier2017} have 
shown that an eccentricity increase can occur from disc--planet interactions when a gap is present in the disk. They confirm the interpretation of \citet{Dangelo2006} that the excited resonance are the 2:4 or 3:5 rather than the 1:3 proposed by \citet{Papaloizou2001}, but haven't assessed the validity of these results numerically. Our idea to explain the eccentricity distrubtion of Jupiter-like planets is therefore already present in the litterature at the linear order. } 

This simple idea is also motivated by observations, as disks with cavities - so called transition disks - have been extensively observed (see e.g., \citet{Calvet2002,Furlan2009,Muzerrolle2010,Hoadley2015,Banzatti2015,Vandermarel2016,Wilson2016,Ercolano2017,Kudo2018,Kluska2018,Gabellini2019} and reviews in \citet{Gorti2016,Ercolano2017-r}) and \citet{Muley2019} even proposed that the shape of PDS70 is due to an eccentric super Jupiter inside the cavity. \cb{I think there is far too many references here!!} Whether the eccentric planet is responsible for the cavity or the cavity for the eccentricity of the planet, however, is not a priori known. 

The paper is organized as follows: in section \ref{sec:description}, we detail the numerical setups we have used to test the effects of migration inside a cavity. We then discuss the results and the effects of different parameters on the growth of eccentricity in section \ref{sec:results}. Finally, we discuss the comparisons of our results with observations and the implications they have for the evolution of protoplanetary disks in section \ref{sec:discussion}. Globally, we do not aim at proposing the most realistic simulation of planet migrating in cavity, but rather exhibiting the fact that the eccentricity growth is a strong feature for such planets, simple and robust in the numerical sense. Eventually we obtain that migration into cavities is a powerful mechanism to pump the eccentricities of giant planets up to the observed values, \corr{without the need for planet--planet scattering}.

% ===============

